Achievable Rates for the General Gaussian Multiple Access Wire-Tap Channel with Collective Secrecy

We consider the General Gaussian Multiple Access Wire-Tap Channel (GGMAC-WT). In this scenario, multiple users communicate with an intended receiver in the presence of an intelligent and informed eavesdropper who is as capable as the intended receiver, but has different channel parameters. We aim to provide perfect secrecy for the transmitters in this multi-access environment. Using Gaussian codebooks, an achievable secrecy region is determined and the power allocation that maximizes the achievable sum-rate is found. Numerical results showing the new rate region are presented. It is shown that the multiple-access nature of the channel may be utilized to allow users with zero single-user secrecy capacity to be able to transmit in perfect secrecy. In addition, a new collaborative scheme is shown that may increase the achievable sum-rate. In this scheme, a user who would not transmit to maximize the sum rate can help another user who (i) has positive secrecy capacity to increase its rate, or (ii) has zero secrecy capacity to achieve a positive secrecy capacity.

==> GGMACWT_ALLERTON06_helpsup.tex <==
\newcommand{\thetadotjJ}{\thetadot^{(j\in\Js)}}
\newcommand{\phiSdotjJ}{\phiSdot^{(j \in \Js)}}
\newcommand{\phiSdotjJc}{\phiSdot^{(j \in \Jsc)}}

We can write \eqref{eqn:ColLagder} out separately for $j \in \Js$ and $j \not \in \Jsc$:
\begin{align}
\frac{\del \Lag_\Js(\Pv,\muv)}{\del P_j} & \\
&\hspace{-1in} =\case
	{\rhodotj(\Pv) \theta_\Js(\Pv)+\rho(\Pv) \thetadotjJ_\Js(\Pv) +\mu_{2j}
		-\sum_{\Ss \subseteq \Jsc} \mu_{3\Ss} \phiSdotjJ(\Pv)}
	{j \in \Js}
	{\rhodotj(\Pv) \theta_\Js(\Pv) -\mu_{1j} + \mu_{2j} 
	-\sum_{\Ss \subseteq \Jsc} \mu_{3\Ss} \phiSdotjJc(\Pv)}
	{j \in \Jsc}
\end{align}
\begin{align}
\label{eqn:thetadotjJdef}
\thetadotjJ_\Js(\Pv) 
	&\triangleq \frac{1+h_j \theta_\Js(\Pv)}{1+\sum_{k \in \Js} h_k P_k} \\
\label{eqn:phiSdotjJdef}
\phiSdotjJ(\Pv) &\triangleq 
	\frac{\sum_{k \in \Ss} P_k}{\paren{1+\sum_{k \in \Js} P_k}^2}
		+\frac{h_j \sum_{k \in \Ss} h_k P_k}{\paren{1+\sum_{k \in \Ssc}h_k P_k}^2}\\
\label{eqn:phiSdotjJcdef}
\phiSdotjJc(\Pv) &\triangleq \case
	{\frac{1}{1+\sum_{k \in \Js} P_k}-\frac{h_j}{1+\sum_{k \in \Ssc}h_k P_k}}
		{j \in \Ss}
	{\frac{h_j \sum_{k \in \Ss} h_k P_k}{\paren{1+\sum_{k \in \Ssc}h_k P_k}^2}}
		{j \not \in \Ss}
\end{align}

==> GGMACWT_ALLERTON06_out.tex <==
\section{Sum Capacity Outer Bound}
In this section, we find an upper bound on the achievable sum rate.  To this end, we start with a few lemmas:

\begin{lemma}
\label{lem:conv1}
Let $\Xm_\Ks = \{\Xm_k\}_{k=1}^2$. Then,
\begin{equation}
R_\Ks \le \ninv I(\Xm_\Ks;\Ym|\Zm) +\nu_n'
\end{equation}
where $\nu_n' \tozero$ as $\e \tozero$ and $n \toinf$.
\end{lemma}

\begin{proof}
Consider the two inequalities:
\begin{gather}
\label{eqn:lemconv11}
H(\Wm_\Ks|\Zm) \ge H(\Wm_\Ks) -\e \ge n R_\Ks -(2n+1) \e \\
\label{eqn:lemconv12}
H(\Wm_\Ks|\Ym,\Zm) \le H(\Wm_\Ks|\Ym) \le n\nu_n
\end{gather}
where \eqref{eqn:lemconv12} follows using Fano's Inequality with $\nu_n \tozero$ as $n \toinf$. Using \eqref{eqn:lemconv11} and \eqref{eqn:lemconv12}, we can write
\begin{align}
n R_\Ks &\le H(\Wm_\Ks)+2n\e\\
	&\le H(\Wm_\Ks|\Zm)+2n\e + \e +n\nu_n-H(\Wm_\Ks|\Ym,\Zm) \\
	&=I(\Wm_\Ks;\Ym|\Zm)+ n(2\e + \frac{\e}{n}+ \nu_n) \\
	&\le I(\Xm_\Ks;\Ym|\Zm)+n \nu_n'
\end{align}
where $\nu_n' = (2 + \ninv) \e + \nu_n$, and we used $\Markov{W_\Ks}{\Xm_\Ks}{\Ym,\Zm}$ in the last step.  Dividing by $n$ completes the proof.
\end{proof}

Using $\Markov{\Ym}{\Xm_{\Ks}}{\Zm}$, we can write
\begin{align}
I(\Xm_{\Ks};\Ym|\Zm) &= H(\Ym|\Zm) - H(\Ym|\Xm_{\Ks},\Zm) \\
	&= H(\Ym|\Zm) - H(\Ym|\Xm_{\Ks}) \\
	&= H(\Ym|\Zm) - \frac{n}{2} \log (2 \pi e) \\
	&= H(\Ym) - I(\Ym;\Zm) - \frac{n}{2} \log(2 \pi e) \\
	&= H(\Ym) - H(\Zm) + H(\Zm|\Ym) - \frac{n}{2} \log(2 \pi e)
\end{align}
 
